Consistency Training with Virtual Adversarial Discrete Perturbation

Consistency training regularizes a model by enforcing predictions of original and perturbed inputs to be similar. Previous studies have proposed various augmentation methods for the perturbation but are limited in that they are agnostic to the training model. Thus, the perturbed samples may not aid in regularization due to their ease of classification from the model. In this context, we propose an augmentation method of adding a discrete noise that would incur the highest divergence between predictions. This virtual adversarial discrete noise obtained by replacing a small portion of tokens while keeping original semantics as much as possible efficiently pushes a training model's decision boundary. Experimental results show that our proposed method outperforms other consistency training baselines with text editing, paraphrasing, or a continuous noise on semi-supervised text classification tasks and a robustness benchmark

==> 07_conclusion.tex <==
\section{Conclusion}


We present \ours, a consistency training with virtual adversarial discrete perturbation.
Unlike other methods, we utilize the gradients information to approximate the samples that would incur the highest divergence from the models' predictions for efficiently pushing the decision boundary.
% We demonstrate our method's superiority in the experiments.

==> 10_validation_score.tex <==

\input{tables/ssl_results_dev}


==> algorithms/ir.tex <==
\setlength{\textfloatsep}{10pt}


\begin{algorithm}[t!]
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwProg{Fn}{Function}{:}{}
\Input{$\text{input sentence}~\mathbf{x}, \text{refinement steps}~S$}
\Output{$\text{perturbed sentence}~\mathbf{\hat{x}}$}
\Fn{Iterative\_Refinements({$\mathbf{x}$, $S$})}{
    \text{// initial perturbation}
    $\text{Get}~\mathbf{I}~\text{randomly with the ratio}~\tau$ 
    $\mathbf{\hat{x}} \gets \vawr{}(\mathbf{\hat{x}}, \mathbf{I})$ \\
    \text{// iterative refinements} \\
    \For{$s \gets 1$ \KwTo $S$}{ 
        $\mathbf{\hat{x}} \gets \vawr{}(\mathbf{\hat{x}}, \mathbf{I})$ \\
        $ \text{Update}~\mathbf{I}~\text{with the least MLM scores}$
    }
}
\Return {$\mathbf{\hat{x}}$}
\caption{\ir{}}
\label{alg:Iterative_Refinements}
\end{algorithm}


==> background.tex <==
% \section{Background}
 
% %  formal definition
 
% \paragraph{Consistency Regularization} Consistency regularization is defined by regularizing the models' predictions to be invariant when the input is perturbed.
% More formally, we can write the loss function as follows:

% \begin{align}
% \label{eq:consistency_regularization}
% \mathcal{L}_{\text{con}}=\sum_{n=1}^{N}D[~p\left(\cdot \mid \mathbf{x}^{n}\right),~p \left(\cdot \mid T\left(\mathbf{x}^{n}\right)\right)] 
% \end{align}

% %  equation explanation 

% \noindent $D[a,b]$ is a non-negative divergence between $a$ and $b$~(e.g., KL-divergence, mean squared error, cross-entropy), 
% $T$ is a transformation~(i.e., perturbation) of the given samples, and $N$ is the number of samples. 
% Occasionally, the term \textit{consistency regularization} is used in the context of semi-supervised learning; however, the method can also be exploited when unlabeled samples are not available by using labeled samples as $\mathbf{x}^n$~\citep{jiang2019smart, liu2020adversarial, asai2020logic}. 
% Hence, $\mathbf{x}^n$ can be both labeled and unlabeled samples.
% % Also, note that the Eq.~\ref{eq:consistency_regularization} only expresses the frame of perturbing the single term~\cite{miyato2018virtual, xie2019unsupervised}. 
% % However, conducting the perturbations on both terms is also possible~\citep{sajjadi2016regularization, berthelot2019remixmatch, sohn2020fixmatch}.

% \begin{figure}[t!]
% \centering
% \resizebox{0.5\textwidth}{!}{
% \includegraphics[width=1\linewidth]{figures/intro_1.png}
% }
% \caption{Given a limited number of labeled samples~(triangles), the training model is prone to overfitting~(left figure). However, when utilizing original and perturbed unlabeled samples~(circles with different colors) by the consistency regularization framework, the training model's decision boundary can be pushed to the low-density region~(right figure). Best viewed in colors.}
% \label{fig:intro}
% \end{figure}

% %  intuition explanation

% When employing the standard training loss function alone, the trained model's decision boundary may traverse through the high-density regime, especially when a limited number of labeled samples are available.
% However, consistency regularization enforces the low-density separation by encouraging invariant prediction for the unlabeled samples' perturbations. 
% Such consistency and small prediction error can be satisfied when the decision boundary traverses a low-density path~\citep{verma2019interpolation}.
% Thus, by exploiting the unlabeled samples' structural information, the method can effectively regularize the training models.
% The intuition is illustrated in Figure \ref{fig:intro}.


% \paragraph{Transformation} Transformation~(i.e., perturbation) of the samples is a central part in consistency training.
% Existing studies actively studied varying perturbation methods~\citep{miyato2016adversarial, clark2018semi, xie2019unsupervised, asai2020logic}.
% \citet{miyato2016adversarial} acquired the continuous virtual adversarial noise, which would distort the self-prediction the most by the second-order approximation of the divergence and iterative power method. 
% Since then, adversarial noise injection to the embedding space has largely been studied~\citep{wang2019robust, jiang2019smart, liu2020adversarial, chen2020seqvat, sano2019effective} for its convenience in applying the method to the various tasks in natural language processing.

% Other lines of works have focused on generating diverse augmentations while preserving semantic coherency. 
% \citet{xie2019unsupervised} mainly utilizes the back-translation, which paraphrases the given sentence by the use of round-trip translations. 
% Other works have utilized the domain-specific knowledge for the transformation~\citep{minervini2018adversarially, li2019logic, asai2020logic}, such as first-order logic.



==> tables/ppl.tex <==
\begin{table}[t!]
\centering
\resizebox{0.45\textwidth}{!}{
\def\arraystretch{0.85}
\begin{tabular}{ l |  c | cccc}
\toprule
\textbf{Type} & \textbf{Original} & \multicolumn{4}{c}{\textbf{Perturbed}} \\
\textbf{Refinement} & N/A & 0 & 1 & 2 & 3    \\ \midrule
\textbf{Perplexity} & 1.42 & 1.87 & 1.78 & 1.68 & 1.67 \\ \bottomrule
\end{tabular}}
\caption{Average perplexity of the original sentences and perturbed sentences during iterative refinement.}
\label{tab:ppl}
\end{table}


==> tables/ssl_results_dev.tex <==
\begin{table*}[h!]
\centering
\resizebox{0.83\textwidth}{!}{
\def\arraystretch{0.7}
\begin{tabular}{ l | ccc | ccc | ccc }
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{AG\_NEWS}} & \multicolumn{3}{c}{\textbf{YAHOO!}} & \multicolumn{3}{c}{\textbf{DBpedia}} \\[1pt] 
& \textit{\textbf{10}}   & \textit{\textbf{200}}  & \textit{\textbf{2500}} & \textit{\textbf{10}}   & \textit{\textbf{200}}  & \textit{\textbf{2500}} & \textit{\textbf{10}}   & \textit{\textbf{200}}   & \textit{\textbf{2500}}   \\ [1pt]\midrule
 BERT~\citep{devlin2019bert}                  & 79.7 & 89.0 & 92.0 & 58.3 & 70.0 & 73.8 & 97.9 & 98.9  & 99.1    \\ [3pt] 
 EDA~\citep{wei2019eda}                       & 84.4 & 89.3 & 92.2 & 61.9 & 70.4 & 73.8 & 98.6 & 98.8  & 99.2    \\ [3pt] 
 VAT~\citep{miyato2016adversarial}            & 82.3 & 89.4 & 92.3 & 62.2 & 70.5 & 74.2 & 98.6 & 98.9  & 99.2    \\ [3pt] 
 VAT + Ent-Min~\citep{miyato2018virtual}      & 82.2 & 89.9 & 92.4 & 64.2 & 70.8 & 74.3 & 98.7 & 99.0  & 99.2    \\ [3pt] 
 UDA~\citep{xie2019unsupervised}              & 84.3 & 88.7 & 92.0 & 61.6 & 70.2 & 73.7 & 98.2 & 98.9  & 99.2    \\ [1pt] \midrule
 VAT-D                                        & 86.6 & 90.3 & 92.5 & 65.2 & 71.5 & 74.2 & 98.5 & 99.0  & 99.2    \\ 
\bottomrule
\end{tabular}}
\caption{Accuracy on the validation data set from the\textsection{\ref{sec:result_ssl}}. We average five different runs with a differently indexed dataset.}
\label{tab:ssl_results_dev}
\end{table*} 

